Theoretical Analysis of Sparse Optimization with Reparameterization, Weight Decay, and Adaptive Learning Rate

Sparse optimization is a fundamental challenge in various practical applications. A popular approach to sparse optimization is $\ell_p$ regularization. However, it may encounter optimization instability due to the unbounded gradients when $0<p<1$. In this paper, we introduce a novel approach to sparse optimization termed ReWA, based on Reparameterization, Weight decay, and Adaptive learning rate. ReWA is closely connected to $\ell_p$-regularization, yet it unveils a distinct optimization landscape that helps mitigate instability issues. Experiments on CIFAR-10 and ImageNet with ResNets demonstrate that ReWA leads to significant sparsity improvements over the $\ell_1$-regularization approach while preserving test accuracy.

==> fig/ell-p.tex <==
\begin{figure}[t]
    \centering
\begin{subfigure}{0.32\textwidth}
\centering
    \begin{tikzpicture}
\begin{axis}[
    % xlabel = $x$,
    % ylabel = $x^p$,
    xmin=-3,
    xmax=3,
    ymin=-0.5,
    ymax=2,
    axis lines=middle, % Show only the x and y axes
    axis line style={-latex, ultra thick}, % Style for the axes lines
    width=\textwidth,
    % height=0.6\textwidth,
    samples=2000,
    xtick=\empty,
    ytick=\empty,
]
\addplot[blue,ultra thick,domain=-3:3] {abs(x)^0.3};
\end{axis}
\end{tikzpicture}
\caption{$\y = \x^{p} \ (0<p<1)$}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\centering
    \begin{tikzpicture}
\begin{axis}[
    % xlabel = $x$,
    % ylabel = $x^p$,
    xmin=-3,
    xmax=3,
    ymin=-0.5,
    ymax=2,
    axis lines=middle, % Show only the x and y axes
    axis line style={-latex, ultra thick}, % Style for the axes lines
    width=\textwidth,
    % height？=0.6\textwidth,
    samples=2000,
    xtick=\empty,
    ytick=\empty,
]
\addplot[blue,ultra thick,domain=-3:-1] {abs(x)^0.3};
\addplot[blue,ultra thick,domain=1:3] {abs(x)^0.3};
\addplot[orange,ultra thick,domain=-1:1] {1};
\addplot[blue,ultra thick,dashed, domain=-1:1] {abs(x)^0.3};
\end{axis}
\end{tikzpicture}
\caption{Constant Clipping}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\centering
    \begin{tikzpicture}
\begin{axis}[
    % xlabel = $x$,
    % ylabel = $x^p$,
    xmin=-3,
    xmax=3,
    ymin=-0.5,
    ymax=2,
    axis lines=middle, % Show only the x and y axes
    axis line style={-latex, ultra thick}, % Style for the axes lines
    width=\textwidth,
    % height=0.6\textwidth,
    samples=2000,
    xtick=\empty,
    ytick=\empty,
]
\addplot[blue,ultra thick,domain=-3:-1] {abs(x)^0.3};
\addplot[blue,ultra thick,domain=1:3] {abs(x)^0.3};
\addplot[orange,ultra thick,domain=-1:1] {0.3*abs(x) + 0.7};
\addplot[blue,ultra thick,dashed, domain=-1:1] {abs(x)^0.3};
\end{axis}
\end{tikzpicture}
\caption{$\ell_1$ Clipping}
\end{subfigure}
    \caption{Clipping for $\ell_p$ regularization. The blue lines (solid and dotted) represent the original $\ell_p$ regularization, and the orange lines represent the clipped version at some clipping point.}
    \label{fig: clipping}
\end{figure}
